Utilizing Free Clients in Federated Learning for Focused Model Enhancement

Federated Learning (FL) is a distributed machine learning approach to learn models on decentralized heterogeneous data, without the need for clients to share their data. Many existing FL approaches assume that all clients have equal importance and construct a global objective based on all clients. We consider a version of FL we call Prioritized FL, where the goal is to learn a weighted mean objective of a subset of clients, designated as priority clients. An important question arises: How do we choose and incentivize well aligned non priority clients to participate in the federation, while discarding misaligned clients? We present FedALIGN (Federated Adaptive Learning with Inclusion of Global Needs) to address this challenge. The algorithm employs a matching strategy that chooses non priority clients based on how similar the models loss is on their data compared to the global data, thereby ensuring the use of non priority client gradients only when it is beneficial for priority clients. This approach ensures mutual benefits as non priority clients are motivated to join when the model performs satisfactorily on their data, and priority clients can utilize their updates and computational resources when their goals align. We present a convergence analysis that quantifies the trade off between client selection and speed of convergence. Our algorithm shows faster convergence and higher test accuracy than baselines for various synthetic and benchmark datasets.

==> bullets.tex <==

% \iscomment{If we go with Indian spelling, shouldn't it be Prioritised?}

% \iscomment{I worry that if we emphasize the ``incentivizing'' in the title/abstract, readers may expect a more explicit incentive policy, more game theoretic or something}

% \begin{itemize}
%     \item Put the context of finding client quality and utility
%     \item Our thing uses loss matching, no low or high loss considerations
%     \item Shakespeare??
%     \item Partial Participation, Non-convex, Need to run for synthetic experiments too
%     \item Homogenization
%     \item Benefit for local clients?? Run experiments comparing the local model of free clients to this global model to show a CLEAR incentive. Want to talk about how a good global model can be used to personalize for local clients
%     \item Polarization of clients as a picture in the intro
%     \item Learning rate tuning
%     \item Change batch size, number of local iterations
%     \item lr fmnist emnist 0.1, cifar 0.01
%     \item Add a bold in the intro talking about incentives
%     \item Implications to fairness
%     \item Look at common implications pointed out 
%     \item Linear speedup??
%     \item Need to renormalise x-axis of graphs with communication rounds
% \end{itemize}
